Intelligent OPC Engineer Assistant for Semiconductor Manufacturing

Advancements in chip design and manufacturing have enabled the processing of complex tasks such as deep learning and natural language processing, paving the way for the development of artificial general intelligence (AGI). AI, on the other hand, can be leveraged to innovate and streamline semiconductor technology from planning and implementation to manufacturing. In this paper, we present \textit{Intelligent OPC Engineer Assistant}, an AI/LLM-powered methodology designed to solve the core manufacturing-aware optimization problem known as optical proximity correction (OPC). The methodology involves a reinforcement learning-based OPC recipe search and a customized multi-modal agent system for recipe summarization. Experiments demonstrate that our methodology can efficiently build OPC recipes on various chip designs with specially handled design topologies, a task that typically requires the full-time effort of OPC engineers with years of experience.

==> doc/checklist.tex <==
\clearpage
\appendix
\onecolumn
\section{Reproducibility Checklist}


\noindent \textbf{This paper:}
\begin{itemize}
  \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes})
  \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{yes})
  \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{yes})
\end{itemize}
\noindent \textbf{Does this paper make theoretical contributions? (\textbf{yes})}
If yes, please complete the list below.
\begin{itemize}
  \item All assumptions and restrictions are stated clearly and formally. (\textbf{yes})
  \item All novel claims are stated formally (e.g., in theorem statements). (\textbf{yes})
  \item Proofs of all novel claims are included. (\textbf{yes})
  \item Proof sketches or intuitions are given for complex and/or novel results. (\textbf{yes})
  \item Appropriate citations to theoretical tools used are given. (\textbf{yes})
  \item All theoretical claims are demonstrated empirically to hold. (\textbf{yes})
  \item All experimental code used to eliminate or disprove claims is included. (\textbf{yes})
\end{itemize}


\noindent \textbf{Does this paper rely on one or more datasets? (\textbf{yes})}
If yes, please complete the list below.
\begin{itemize}
  \item A motivation is given for why the experiments are conducted on the selected datasets (\textbf{yes})
  \item All novel datasets introduced in this paper are included in a data appendix. (\textbf{yes})
  \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textbf{yes})
  \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textbf{yes})
  \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\textbf{yes})
\end{itemize}


\noindent \textbf{Does this paper include computational experiments? (\textbf{yes})}
If yes, please complete the list below.
\begin{itemize}
  \item Any code required for pre-processing data is included in the appendix. (\textbf{yes}).
  \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{yes})
  \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes})
  \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{yes})
  \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{yes})
  \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{yes})
  \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes})
  \item This paper states the number of algorithm runs used to compute each reported result. (\textbf{yes})
  \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{yes})
  \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\textbf{yes})
  \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{yes})
  \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{yes})
\end{itemize}

==> doc/rl1.tex <==

The RL framework for OPC recipe generation is modeled as a Markov Decision Process (MDP), defined by the tuple $(\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R})$:

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.98\linewidth]{opc/opc_engine/rl.pdf}
  \caption{Reinforcement Learning for Global OPC Optimization.}
  \label{fig:rl_framework}
\end{figure}

\begin{itemize}
    \item $\mathcal{S}$: State space, representing the positions of the segmentation points along the edges of the polygon.
    \item $\mathcal{A}$: Action space, consisting of three types of actions:
    % \begin{enumerate}
1) Change corner length.
2) Move segmentation points within fragments.
3) Adjust EPE measurement points.
    % \end{enumerate}
    \item $\mathcal{P}$: State transition probabilities, denoted as $\mathcal{P}(s_{t+1} \mid s_t, a_t)$, which define the probability of transitioning to state $s_{t+1}$ from state $s_t$ when action $a_t$ is taken.
    \item $\mathcal{R}$: Reward function, $R(s_t, a_t)$, based on the errors between the printed image and the design.
\end{itemize}

\subsubsection{State and Action Representation}

The environment is the layout, typically represented in formats such as GDS or OASII in the semiconductor industry, abstracted as polygons. The state $s_t \in \mathcal{S}$ at time $t$ is defined by the positions of the segmentation points along the polygon edges.
The action $a_t \in \mathcal{A}$ at time $t$ can be one of the following:
% \begin{enumerate}
1) Adjust the length of the corner segments.
2) Move the position of intermediate segmentation points within fragments.
3) Change the position of EPE measurement points.
% \end{enumerate}

\subsubsection{Reward Function}
The reward $R_t$ is calculated based on the lithography simulation results after applying DiffOPC to the layout. The printed image is compared to the design image, generating the following errors:
% \begin{itemize}
$L2$ error ($\mathcal{L}_2$);
Process variation band error ($\mathcal{L}_{\text{PVB}}$);
Edge placement error (EPE) ($\mathcal{L}_{\text{EPE}}$).
% \end{itemize}
The reward $R_t$ is the negative sum of these errors, encouraging the minimization of discrepancies between the printed and design images:
\begin{equation}
R_t = - \left( \mathcal{L}_2 + \mathcal{L}_{\text{PVB}} + \mathcal{L}_{\text{EPE}} \right)
\end{equation}

\subsubsection{Algorithm Workflow}
The algorithm follows a standard RL loop:
\begin{enumerate}
    \item \textbf{Initialization}: Start with an initial layout and segmentation points $s_0$.
    \item \textbf{Action Selection}: The agent selects an action $a_t$ based on the current state $s_t$, typically using a policy $\pi(a_t \mid s_t)$.
    \item \textbf{State Transition}: The environment transitions to a new state $s_{t+1}$ according to the state transition probability $\mathcal{P}(s_{t+1} \mid s_t, a_t)$.
    \item \textbf{Reward Calculation}: The reward $R_{t+1}$ is computed based on the new layout after applying DiffOPC.
    \item \textbf{Policy Update}: The agent updates its policy $\pi$ based on the reward and the new state, often using algorithms such as Q-learning, SARSA, or policy gradient methods.
\end{enumerate}


\todo{Change to PPO.}
\subsubsection{Mathematical Formulation}

The goal of the RL agent is to find an optimal policy $\pi^*$ that maximizes the expected cumulative reward, defined as the return $G_t$:
\begin{equation}
G_t = \sum_{k=0}^{\infty} \gamma^k R_{t+k+1},
\end{equation}
where $\gamma$ is the discount factor.
The action-value function $Q^\pi(s, a)$ represents the expected return for taking action $a$ in state $s$ under policy $\pi$:
\begin{equation}
Q^\pi(s, a) = \mathbb{E} \left[ G_t \mid s_t = s, a_t = a \right].
\end{equation}
The optimal action-value function $Q^*(s, a)$ satisfies the Bellman equation:
\begin{equation}
Q^*(s, a) = \mathbb{E} \left[ R_{t+1} + \gamma \max_{a'} Q^*(s_{t+1}, a') \mid s_t = s, a_t = a \right].
\end{equation}
The optimal policy $\pi^*$ selects actions that maximize $Q^*(s, a)$:
\begin{equation}
\pi^*(s) = \arg\max_{a} Q^*(s, a).
\end{equation}

% \subsubsection{Conclusion}

% By leveraging RL, the OPC recipe generation process can be automated, exploring a vast parameter space to identify optimal fragment configurations. This approach reduces manual tuning efforts and enhances the precision of lithography simulations.


